3D Face Tracking from 2D Video through Iterative Dense UV to Image Flow

When working with 3D facial data, improving fidelity and avoiding the uncanny valley effect is critically dependent on accurate 3D facial performance capture. Because such methods are expensive and due to the widespread availability of 2D videos, recent methods have focused on how to perform monocular 3D face tracking. However, these methods often fall short in capturing precise facial movements due to limitations in their network architecture, training, and evaluation processes. Addressing these challenges, we propose a novel face tracker, FlowFace, that introduces an innovative 2D alignment network for dense per-vertex alignment. Unlike prior work, FlowFace is trained on high-quality 3D scan annotations rather than weak supervision or synthetic data. Our 3D model fitting module jointly fits a 3D face model from one or many observations, integrating existing neutral shape priors for enhanced identity and expression disentanglement and per-vertex deformations for detailed facial feature reconstruction. Additionally, we propose a novel metric and benchmark for assessing tracking accuracy. Our method exhibits superior performance on both custom and publicly available benchmarks. We further validate the effectiveness of our tracker by generating high-quality 3D data from 2D videos, which leads to performance gains on downstream tasks.

==> figures/mq/multiface_quantitative_old.tex <==

\begin{table*}[th]
\tablefont
\setlength{\tabcolsep}{4pt}
\label{tab:multiface_benchmark_no_temporal}
% \begin{center}
\begin{tabular}{ l|c c c c c|c c c c c } 
\multicolumn{11}{l}{\textbf{No temporal information sharing (single image)}} \\
\hline
\multirow{2}*{Method} & \multicolumn{5}{c|}{CD (mm) $\downarrow$} & \multicolumn{5}{c}{$\overline{\text{SSME}}$ (px) $\downarrow$}  \\[2pt]
\cline{2-11}
                & face   & mouth  & eyes   & nose   & ears   & face   & mouth  & eyes   & nose   & ears \\
\hline
         DECA   & 1.37 &    1.29 &    1.32 &    1.08 &    2.68 &    5.66 &    6.16 &    3.60 &    4.25 &    8.34 \\
         EMOCA  & 1.47 &    1.46 &    1.49 &    1.10 &    2.71 &    6.14 &    7.32 &    3.99 &    4.26 &    8.55 \\
          HRN   & 1.49 &    1.39 &    1.24 &    1.09 &       - &    5.75 &    6.04 &    4.20 &    4.84 &       - \\
      3DDFAv2   & 1.53 &    1.52 &    1.59 &    1.24 &       - &    7.91 &    9.47 &    6.65 &    6.55 &       - \\
        PRNet   & 1.55 &    1.59 &    1.50 &    1.28 &       - &    8.45 &   10.66 &    5.98 &    6.03 &       - \\
      SADRNet   & 1.49 &    1.52 &    1.49 &    1.22 &       - &    7.11 &    8.21 &    5.15 &    5.53 &       - \\
         Ours   & 1.22 &    1.25 &    1.10 &    1.01 &    2.33 &    2.85 &    3.32 &    1.46 &    2.21 &    2.10 \\
\hline
\end{tabular}
% \end{center}
\caption{Results on our Multiface tracking benchmark without and without temporal information sharing. }
\end{table*}


\begin{table*}[t]
\tablefont
\label{tab:multiface_benchmark_with_temporal}
\begin{center}
\begin{tabular}{ l|c c c c c|c c c c c } 
\multicolumn{11}{l}{\textbf{With temporal information sharing (sequence)}} \\
\hline
\multirow{2}*{Method} & \multicolumn{5}{c|}{CD (mm) $\downarrow$} & \multicolumn{5}{c}{$\overline{\text{SSME}}$ (px) $\downarrow$}  \\ 
\cline{2-11}
              &    face &   mouth &    nose &    eyes &    ears &    face &   mouth &    nose &    eyes &    ears \\
\hline
         DECA &    1.37 &    1.29 &    1.32 &    1.08 &    2.68 &    5.26 &    6.12 &    3.22 &    3.87 &    7.10 \\
        EMOCA &    1.47 &    1.46 &    1.49 &    1.10 &    2.71 &    5.63 &    6.95 &    3.56 &    3.87 &    7.28 \\
          HRN &    1.49 &    1.39 &    1.24 &    1.09 &       - &    4.63 &    5.39 &    3.02 &    3.68 &       - \\
      3DDFAv2 &    1.53 &    1.52 &    1.59 &    1.24 &       - &    6.71 &    8.43 &    5.43 &    5.44 &       - \\
        PRNet &    1.55 &    1.59 &    1.50 &    1.28 &       - &    7.54 &    9.80 &    5.25 &    5.35 &       - \\
      SADRNet &    1.49 &    1.52 &    1.49 &    1.22 &       - &    6.18 &    7.46 &    4.31 &    4.72 &       - \\
          MPT &    1.30 &    1.47 &    1.11 &    0.96 &       - &    5.74 &    7.34 &    4.64 &    4.01 &       - \\
         Ours &    1.22 &    1.25 &    1.10 &    1.01 &    2.33 &    2.85 &    3.32 &    1.46 &    2.21 &    2.10 \\
\hline
\end{tabular}
\end{center}
\caption{Results on our Multiface tracking benchmark with temporal information sharing. }
% Smoothing is applied to single view methods
\end{table*}

==> sec/X_coverpage.tex <==
\section*{Comment Formats}

\noindent \commentmat{This is a comment by Mat}\\
\commentft{This is a comment by Felix}\\

\section*{General Formatting Commands}
\noindent \added{this is newly added text, for review}\\
\remove{this is text someone things should be removed}\\
\maybe{this is text added/modified, with a "maybe". not sure.}\\
\alt{this is alternative text, to the previous sentence or paragraph or something}

\section*{Page Layouts}
\noindent - 8 page total, not including (1) references (2) appendix \\
- Section we need to have include: Abstract, Introduction, Background, Key Insight, Method, Experiments, Related Work, Conclusion
\begin{itemize}
    \item $1.5$ pages: Abstract + Introduction
    \item $1$ pages: Background
    \item $\sim 2/3$ page: Key Insight
    \item $1.5$ pages: Method 
    \item $2$ pages: Experiments
    \item $0.5$ pages: Related Works
    \item $\sim 1/3$ pages: Conclusion
\end{itemize}

\section*{The Story}
\begin{itemize}
    \item This topic is neglected far and wide
    \begin{itemize}
        \item Many fields use 3D face trackers, yet little attention is given to this task
    \end{itemize}
    \item This problem is "defined" as the 3D face tracking from videos. We are reconstructing 3D faces from single view. \todo{is there a formal definition?}
    \item In tandem, there are 3 subtasks that need to be decoupled:
    \begin{enumerate}
        \item Face pose
        \item Shape
        \item Expression
    \end{enumerate}
    \item \todo{does OpenPose fit in here somewhere?}
    \item Few works actually perform the above decoupling, and there are no benchmarks to test on: all the benchmarks focus on 3D reconstruction, but the motion isn't captured (pose evaluation is wrong)
    \begin{itemize}
        \item Similarly, the motion along tangents is wholistically ignored (not calculated right) \todo{need examples}
        \item Or, the evaluation is on sparse landmarks which cannot be defined absolute for all faces. This has practical limitations and introduces sources of error
    \end{itemize} 
    \item We tackle all the above with our metric. As well, we develop a pipeline for training and evaluations for this \todo{dense} motion
    \item We also develop a new training set around this new paradigms
    \begin{itemize}
        \item new keypoint detector
        \item new metric
    \end{itemize}
    \item We want to push this research into this new direction that we believe is better
    \item Existing works only rely on photometric approaches, and doesn't train or eval on this "dense deformation"
    \item Microsoft has some new work on synthetic data
    \begin{itemize}
        \item but it's still landmarks: and who defines these landmarks? where exactly on the eyebrow does it go? it's impossible to apply in a practical setting
        \item motion is practically impossible to evaluate/measure in this setting
    \end{itemize}
    \item But, optical flow can do these things, that's why we evaluate on it and develop this metric.
    \item Our method is also invariant to camera models, intrinsics, face shape, pose, etc.
    \item This tracking problem using sparse landmarks is ill-posed, and our metric alleviates that problem in many ways
\end{itemize}

\newpage
